Iroko: A Framework to Prototype Reinforcement Learning for Data Center Traffic Control

Recent networking research has identified that data-driven congestion control (CC) can be more efficient than traditional CC in TCP. Deep reinforcement learning (RL), in particular, has the potential to learn optimal network policies. However, RL suffers from instability and over-fitting, deficiencies which so far render it unacceptable for use in datacenter networks. In this paper, we analyze the requirements for RL to succeed in the datacenter context. We present a new emulator, Iroko, which we developed to support different network topologies, congestion control algorithms, and deployment scenarios. Iroko interfaces with the OpenAI gym toolkit, which allows for fast and fair evaluation of different RL and traditional CC algorithms under the same conditions. We present initial benchmarks on three deep RL algorithms compared to TCP New Vegas and DCTCP. Our results show that these algorithms are able to learn a CC policy which exceeds the performance of TCP New Vegas on a dumbbell and fat-tree topology. We make our emulator open-source and publicly available: https://github.com/dcgym/iroko

==> challenges.tex <==
 \section{Challenges}

 \subsection{Scale}
 In terms of data collection and compute cost we assume the same scalability 
 properties as FastPass, which relies on a DPDK-enhanced~\cite{dpdk} arbiter on 
 an eight-core 10GB NIC machine.

 A traffic matrix with many features and many nodes will generate a large state 
 space.
 However, if the controller is intended to manage independent data center pods 
 only, the state space is manageable.
 Using the Facebook's Altoona~\cite{fb_dc} datacenter as an example, one pod is 
 comprised of approximately 768 end nodes and 52 switches, each with 48 ports.
 This adds up to a size of ~7488 (2496 switch ports * 3 features) states. Data 
 size increases drastically the more features are added. As of now, we consider 
 queue length, utilization and the flow hash to be sufficient.

 Assuming an MTU data request/reply size of 1500 bytes and a (very 
 aggressive) query epoch of 1 ms, a single 10GB NIC can serve approximately 800 
 network elements per millisecond. This can easily be scaled up using more 
 capable interface cards and multiple 
 interfaces.


==> rl_dc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{RL in the Datacenter}
\label{sec:proposal}

\subsection{Learning}
Before the agent can ever be effective, it has to be trained on real 
traffic first. This may either happen offline, by performing supervised 
learning on real traces, or online using off-policy iteration. Here, the 
controller observes the operation of a default datacenter for an arbitrary 
amount of time until it converges to a policy that is satisfactory. A similar 
model is used in the training of deep-learning frameworks such as AlphaGo 
Zero~\cite{alphago} or Atari agents~\cite{dq_learning}.
Once the agent's policy is trained, it can be deployed in the 
datacenter.

\subsection{Decentralized vs Centralized Control}

\subsubsection{Decentralized Agents}

A decentralized agent offers the advantage of scalability and reliability, as 
individual failures will not affect the entire system state.

Adaptive end-to-end algorithms such as PCC~\cite{pcc} and Copa~\cite{copa} 
%TODO Copa needs to be verified
already propose self-optimization, but do so only locally on the end host, 
where the algorithm maximizes its own utility and eventually converges.
These approaches have been designed with the Internet in 
mind, where fairness and eventual convergence are necessities. In the data 
center, the prevalence of short, bursty flows and very low RTT often limits 
convergence, leading to inefficient flow utilization or instantaneous queue 
build up.

\subsubsection{Central Agents}
Adhering to the conventional SDN network architecture, a central autonomous 
arbiter can manage nodes based on its current optimal network model.
It periodically queries switches or hosts to update its global view and 
executes actions based on this information. It learns by observing the network 
state feedback and continuously updates its action policy.
This agent can follow the proactive congestion control school of 
thought~\cite{perc}. 
Instead of responding to network feedback, it plans ahead and asynchronously 
grants hosts traffic guarantees based on its current anticipated optimal model 
of the network.

The central, managed approach has several advantages. First, the controller 
acts as a propagator of global optimal information, which it can disseminate 
across the network in the form of actions and sending rate policies. %awkward 
%sentence
Secondly, the agent acts as an interface between the concrete reinforcement 
learning algorithm and the data center. Concrete datacenter information is 
abstracted away from the algorithm, providing flexibility in data acquisition 
and modeling.
Thirdly, the major concern of signalling latency delay of central scheduling 
systems is mitigated by operating asynchronously and predictively.
In an ideal word, events in epoch $e_t+2$ are already anticipated for in 
$e_{t}$ and precautions have been executed in $e_{t+1}$.
% The arguments here need to be stronger
\subsection{Defining the Environment}
Another fundamental challenge is to formalize what the agent "sees", i.e., how 
the environment of the data center is abstracted. The available options of data 
acquisition in a DC are manifold, ranging from simple switch statistics, to 
application flows, job deployment monitoring, or even explicit application 
notifications. The agent can predict localized surges of traffic from an 
incoming job request or flow pattern and execute anticipatory actions to soften 
the impact.
Ideally, the central controller should have knowledge about all activities in 
the data center to infer traffic correlations. This may be infeasible due 
to constraints in security as well as hardware monitoring. In this work, we 
focus on the transport layer. The agent remains independent of higher layer 
applications and only operates based on its view of the global datacenter. 
%\ugh{Should probably mention the Eden paper here}
 Modeling an objective function based only on congestion signals is a tried 
and tested approach. Remy~\cite{remy} and PCC~\cite{pcc} have demonstrated 
that it is possible to dynamically learn and improve the congestion function 
on simple network feedback.
 
We assume that the arbiter is fed a $nxd$ traffic matrix which models the data 
center as a list of $n$ ports $n$ with $d$ network features.
Even on the transport level, the possible feature set is diverse. 
The agent acts as authorized manager of the network and is 
theoretically able to query switch buffer occupancy, packet drops, 
port utilization, active flows, round-trip time (RTT), end-hosts, etc. All of 
these attributes play a part in the accurate identification of patterns.

%Similar to the feedback functionality in TCP, the dynamic environment will 
%serve as the input of the reward model for the agent.

One viable approach is to only use switch buffer occupancy\footnote{We assume 
that switches are capable of reliably providing these statistics.}, interface 
utilization, and active flows as a target environment. 
Increasing RTT has been used effectively as a congestion signal in congestion 
work~\cite{timely}.
%\ugh{Maybe more paper references} 
Queue length is a discrete value and precedes the impact of RTT, making it an 
equivalent congestion signal metric. Utilization serves as a regularization 
parameter to avoid optimizing only for minimum queue size (and easy solution 
for zero queue would be to not send at all). Finally, a hash of active TCP/UDP 
flows serves as basis to identify network patterns.
The reinforcement agent is able to periodically query these statistics from 
switches in the network, which it stores as the $dxn$ traffic matrix. 
The matrix updates on the scale of a few milliseconds, which is sufficient to 
sample the majority of flows~\cite{fb_dc}. 
\subsubsection{Scale}

A traffic matrix with many features and many nodes will generate a large state 
space, which is possibly even continuous if link bandwidth is to be monitored.
However, if the controller is intended to manage independent data center pods 
only, the state space is manageable. 
Using the Facebook's Altoona~\cite{fb_dc} datacenter as an example, one pod is 
comprised of approximately 768 end nodes and 52 switches, each with 48 ports. 
This adds up to a size of ~7488 (2496 switchports * 3 features) states. Data 
size increases drastically the more features are added. As of now, we consider 
queue length, utilization and the flow hash to be sufficient.

As seen in Section~\ref{sec:rl} approximating large state space is a well known 
problem in the field of reinforcement learning.
%\ugh{Michael, what are good papers to add here? DDPG, FPS, DOTA?, 
%Self-Driving?}.
Techniques typically include the use of neural networks to reduce the amount of 
compute needed.
In terms of data collection and compute cost we assume the same scalability 
properties as FastPass, which relies on a DPDK-enhanced~\cite{dpdk} arbiter on 
an eight-core 10GB NIC machine.
Assuming an MTU data request/reply size of 1500 bytes and a (very 
aggressive) query epoch of 1 ms, a single 10GB NIC can serve approximately 800 
network elements per millisecond.
%\ugh{Would be good to have a substantial citation here}
This can easily be scaled up using more capable interface cards and multiple 
interfaces. We discuss more scalability issues in section \ref{sec:challenges}.


\subsection{Congestion Feedback}
Corresponding to the modeling of the state space, the agent requires a concrete 
objective to optimize for. This object may be any goal the network operator 
defines. Finding the right objective function is crucial for the agent to 
succeed and defines the success of the model. 


In this work, our model targets the minimization of bufferbloat in the network. 
We roughly follow a common trade-off model, inspired by recent work on TCP 
congestion control optimization~\cite{learning_tcp}:
\begin{equation}
\delta *(\text{throughput}_{cur}) - \text{queue}_{cur}
\end{equation}
where \textit{throughput} describes the current throughput, \textit{queue} the 
current queue size of switch ports, and $\delta$ the 
weight of bandwidth maximization relative to maximum queue length and bandwidth.
A reduction in overall queue length in the coming epochs signals a 
positive reward for the agent. Such a naive approach raises two major concerns: 
overfitting (no sending == no queue buildup) and the credit assignment problem 
(How do we now our actions and not random chance caused the buffer reduction?)

The overfitting is reduced by using network utilization as regularization 
parameter. Agents continuously increase available bandwidth for end-hosts until 
queuing occurs, which acts as a penalty. Correspondingly, if queuing decreases 
but bandwidth does too, reward is diminished.

In terms of positive feedback (queuing is reduced but bandwidth remains 
constant) we rely neural net backpropagation to appropriately 
assign rewards to actions.
% \ugh{Michael, do we have a good paper on that space other than the typical 
%DDPG stuff?} 

Alternatives to this approach may also include reports by hosts on flow 
completion times, latency, or retransmits.
If applications are starving or are continuously over-allocated, they can 
signal the agent, which incorporates the feedback into its reward function.


\subsection{Choosing the Actions}
% Not sure if we should talk about load balancing still.
Solutions in datacenter congestion control boil down to four major categories. 
%\ugh{dangerous statement}
Load-balancing (routing/switching), sending rate 
adjustment (SAR), queue management, and explicit hardware modification. 
We focus on the first two categories. Explicit modification is unlikely for a 
software controller and we intend to eliminate queues entirely. Queue 
management is thus orthogonal to our work.

\subsubsection{Load-balancing}\label{sec:loadbalance}
One action option for the agent is to balance traffic across the datacenter to 
unclog bottlenecks and maximize link utilization. This technique has 
demonstrated success many times in different 
shapes~\cite{hedera,microte,conga,learning_route,antnet}. % Check these papers 
%properly.

Central controllers are able to quickly recognize elephant flows or 
bursts and reroute traffic in the right time, whereas local load-balancing 
techniques or multi-path schemes scatter packets across many links. However, 
load-balancing is merely a mitigation technique to deal with suboptimal traffic 
distribution and does not address the underlying issue of excess sending rate.
A controller shifting traffic routes and flows can only do so much to keep 
traffic bursts and buffer overflow under control. In addition, the network 
impact of a wrong routing decision is substantially higher than suboptimal 
rate-limiting (host starvation). Load-balancing should thus be considered much 
more carefully in a reinforcement learning setting.

Instead, we propose to tackle the root of the cause of congestion, which is 
excess sending rate and lack of fast convergence to an optimum. 
Note that we do not believe that these action sets should be exclusive. 
Reinforcement Learning has already been discussed in the context of route 
optimization~\cite{antnet,learning_route}. In 
fact, it is much more beneficial to optimize both routing as well as 
traffic control. We agree with the proposal of DeepConfig~\cite{deepconfig} 
that a multi-agent system should manage the network completely 
autonomously.
For now, we view such a multi-agent system to be out of scope and focus 
on a model for fine-grained traffic limiting instead.

\subsubsection{SAR}
Remote SAR can be expressed in varying granularity, from the flow to the 
switch-level. Ideally, our agent would model every single flow 
in the network to guarantee an optimum. This, however, is infeasible, as 
accounting for short bursty flows and isolated transmissions (a substantial 
port of flows in datacenter~\cite{fb_dc,msr_dc}) would increase the 
management complexity of the controller dramatically. Instead, we advocate to 
rate-limit on a per-interface basis, and provide each host with a minimum 
guarantee of safe transmit. Instead of operating on the full bandwidth provided 
by the interface a host is just able to send on a subset. The controller 
guarantees that the host will not experience latency increases or loss on this 
subset. The host itself still retains the capability to optimize flows locally, 
and spreads bandwidth allocation per flow based on demand or priority.


A major feature of the controller is that it computes the optimal model 
\textit{asynchronously} and anticipatory.
It periodically broadcasts a bandwidth function which models the host bandwidth 
for $n$ epochs.
The controller will dynamically adjust rate allocations to ensure that 
starving hosts are given more bandwidth , while hosts that are 
overprovisioned have their allocated bandwidth reduced.
This decouples controller compute from the clients and gives breathing room for 
failure handling and fall-back mechanisms.
%~\ugh{Should probably name some, or do we cover that in the challenges 
%section.}
The planning also guarantees that the network remains stable. In the case of 
arbiter failures, hosts simple operate on their given function until 
expiration. Either way, to avoid starving, interfaces are guaranteed a minimum 
bandwidth rate which can be adjusted by the network operator depending on their 
bisection bandwidth and incast tolerance. 

This allocation scheme can be extended to a maximum per-path basis for hosts, 
but will have to be carefully modeled to avoid action-space explosion. We leave 
this feature as future work.
In the ideal instantiation of this system, packet-loss will only rarely, if 
ever, occur. We aim to trade off maximum bandwidth utilization for optimal 
system stability and reliable latency.




